New Constraints on the Galactic Bar

Previous work has related the Galactic Bar to structure in the local stellar velocity distribution. Here we show that the Bar also influences the spatial gradients of the velocity vector via the Oort constants. By numerical integration of test-particles we simulate measurements of the Oort C value in a gravitational potential including the Galactic Bar. We account for the observed trend that C is increasingly negative for stars with higher velocity dispersion. By comparing measurements of C with our simulations we improve on previous models of the Bar, estimating that the Bar pattern speed is Omega_b/Omega_0=1.87\pm0.04, where Omega_0 is the local circular frequency, and the Bar angle lies within 20<phi_0<45 deg. We find that the Galactic Bar affects measurements of the Oort constants A and B less than ~2 km/s/kpc for the hot stars.

==> tab1.tex <==
\begin{deluxetable}{lcc}
\tablewidth{0pt}
\tablecaption{Simulation parameters used\label{table:par}}
\tablehead{
\colhead{Parameter}                  &
\colhead{Symbol}                    &
\colhead{Value}           
} 
\startdata
Solar neighborhood radius   & $r_0$  &   1                            \\
Circular velocity at $r_0$  & $v_0$  &   1                            \\
Radial velocity dispersion & $\sigma_{\rm u}(r_0)$ & $0.05v_0$ or $0.18v_0$ \\
$\sigma_{\rm u}$ scale length & $r_{\sigma}$ & $0.9r_0$                     \\
Disk scale length &  $r_\rho$       &    $0.37r_0$                    \\
Bar strength      &  $\epsilon_{\rm b}$   &     $-0.012$              \\
Bar size          &   $r_{\rm b}$         &     $0.8r_{\rm cr}$
\enddata 
\end{deluxetable}

